Application of Graph Convolutions in a Lightweight Model for Skeletal Human Motion Forecasting

Prediction of movements is essential for successful cooperation with intelligent systems. We propose a model that integrates organized spatial information as given through the moving body's skeletal structure. This inherent structure is exploited in our model through application of Graph Convolutions and we demonstrate how this allows leveraging the structured spatial information into competitive predictions that are based on a lightweight model that requires a comparatively small number of parameters.

==> Tables/quantitative_forecasting_quaternet.tex <==
\begin{table}[h]
    \centering
    \caption{Quantitative results on the motion forecasting task under the evaluation protocol of \cite{quaternet}. The values correspond to the average taken over 128 samples.}
    \label{tab:quantitative_forecasting_quaternet}
    %\scalebox{0.8}{
    \resizebox{\textwidth}{!}{
    \tabcolsep=0.11cm
    \begin{tabular}{l llll l llll l llll l llll}
    \hline
                              & \multicolumn{4}{l}{Walking} & & \multicolumn{4}{l}{Eating} & & \multicolumn{4}{l}{Smoking} & & \multicolumn{4}{l}{Discussion} \\ \cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
               Milliseconds   & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400   & & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400  \\ \toprule
        Run.-avg. 4           & 0.64 & 0.92 & 1.30 & 1.39   & & 0.46 & 0.69 & 0.98 & 1.09  & & 0.48 & 0.67 & 1.02 & 1.14   & & 0.74 & 1.00 & 1.35 & 1.46 \\ 
        Run.-avg. 2           & 0.51 & 0.83 & 1.26 & 1.36   & & 0.35 & 0.63 & 0.95 & 1.07  & & 0.37 & 0.59 & 0.96 & \textit{1.08}   & & 0.60 & 0.90 & 1.31 & 1.45 \\ 
        Zero-velocity         & 0.43 & 0.78 & 1.23 & 1.34   & & 0.30 & 0.59 & 0.94 & 1.07  & & 0.34 & 0.56 & 0.94 & \textit{1.08}   & & 0.55 & 0.83 & 1.27 & 1.46 \\
        GRU unsup.            & 0.34 & 0.61 & 0.92 & 1.02   & & 0.32 & 0.60 & 0.92 & 1.05  & & 0.43 & 0.79 & 1.15 & 1.31   & & 0.57 & 0.88 & 1.34 & 1.48 \\
        OuaterNet vel.        & \textit{0.28} & \textit{0.49} & \textit{0.76} & \textit{0.83}   & & \textbf{0.22} & \textit{0.47} & \textit{0.76} & \textit{0.88}  & & \textit{0.28} & \textit{0.47} & \textit{0.79} & \textbf{0.91}   & & \textit{0.48} & \textit{0.74} & \textit{1.20} & \textit{1.37} \\ \hdashline
    Ours               & \textbf{0.26} & \textbf{0.46} & \textbf{0.73} & \textbf{0.81}   & & \textit{0.24} & \textbf{0.42} & \textbf{0.72} & \textbf{0.84}  & & \textbf{0.25} & \textbf{0.42} & \textbf{0.78} & \textbf{0.91}   & & \textbf{0.40} & \textbf{0.70} & \textbf{1.12} & \textbf{1.30} \\
%    Joint-level \textit{abs.} & 0.33 & 0.54 & 0.82 & 0.94   & & 0.27 & 0.49 & 0.78 & 0.91  & & 0.29 & 0.46 & 0.76 & 0.89   & & 0.44 & 0.72 & 1.17 & 1.36 \\ 

    \hline
                              & \multicolumn{4}{l}{Directions} & & \multicolumn{4}{l}{Greeting} & & \multicolumn{4}{l}{Phoning} & & \multicolumn{4}{l}{Posing} \\ \cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
               Milliseconds   & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400   & & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400  \\ \toprule
        Run.-avg. 4           & 0.46 & 0.67 & 0.99 & 1.14   & & 0.94 & 1.20 & 1.56 & 1.69  & & 0.60 & 0.84 & 1.23 & 1.37   & & 0.64 & 0.93 & 1.35 & 1.54 \\ 
        Run.-avg. 2           & 0.36 & 0.59 & 0.95 & 1.10   & & 0.78 & 1.10 & 1.51 & 1.66  & & 0.48 & 0.75 & 1.18 & 1.33   & & 0.50 & 0.82 & 1.29 & 1.48 \\ 
        Zero-velocity         & 0.30 & 0.54 & 0.92 & 1.08   & & 0.67 & 1.03 & 1.47 & 1.66  & & 0.42 & 0.71 & 1.17 & 1.31   & & 0.42 & 0.75 & 1.25 & 1.45 \\
        GRU unsup.            & 0.32 & 0.58 & 0.98 & 1.15   & & 0.66 & 0.98 & 1.41 & 1.55  & & 0.43 & 0.71 & 1.14 & 1.31   & & 0.47 & 0.84 & 1.39 & 1.58 \\
        OuaterNet vel.        & \textit{0.24} & \textit{0.46} & \textit{0.84} & \textit{1.01}   & & \textit{0.61} & \textit{0.93} & \textit{1.34} & \textit{1.51}  & & \textit{0.36} & \textit{0.61} & \textit{0.98} & \textit{1.14}   & & \textit{0.38} & \textit{0.71} & \textit{1.20} & \textit{1.39} \\ \hdashline
    Ours               & \textbf{0.20} & \textbf{0.40} & \textbf{0.76} & \textbf{0.93}   & & \textbf{0.47} & \textbf{0.75} & \textbf{1.23} & \textbf{1.40}  & & \textbf{0.32} & \textbf{0.55} & \textbf{0.91} & \textbf{1.06}   & & \textbf{0.32} & \textbf{0.61} & \textbf{1.08} & \textbf{1.27} \\
%    Joint-level \textit{abs.} & 0.25 & 0.44 & 0.82 & 0.98   & & 0.50 & 0.81 & 1.24 & 1.43  & & 0.35 & 0.59 & 0.96 & 1.13   & & 0.38 & 0.68 & 1.11 & 1.31 \\
    \hline
                              & \multicolumn{4}{l}{Purchases} & & \multicolumn{4}{l}{Sitting} & & \multicolumn{4}{l}{Sittingdown} & & \multicolumn{4}{l}{Takingphoto} \\ \cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
               Milliseconds   & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400   & & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400  \\ \toprule
        Run.-avg. 4           & 0.80 & 1.09 & 1.41 & 1.50   & & 0.57 & 0.81 & 1.15 & 1.28  & & 0.72 & 1.01 & 1.45 & 1.62   & & 0.39 & 0.54 & 0.80 & 0.90 \\ 
        Run.-avg. 2           & 0.66 & 1.01 & 1.38 & 1.47   & & 0.45 & 0.71 & 1.09 & 1.22  & & 0.59 & 0.90 & 1.37 & 1.54   & & 0.31 & 0.48 & 0.75 & 0.87 \\ 
        Zero-velocity         & 0.56 & 0.95 & 1.37 & \textit{1.46}   & & 0.36 & 0.64 & 1.05 & 1.19  & & 0.52 & 0.88 & 1.38 & 1.57   & & 0.27 & 0.46 & 0.77 & 0.88 \\ 
        GRU unsup.            & 0.57 & 0.97 & 1.38 & 1.48   & & 0.42 & 0.77 & 1.24 & 1.43  & & 0.60 & 1.03 & 1.68 & 1.92   & & 0.31 & 0.53 & 0.90 & 1.06 \\
        OuaterNet vel.        & \textit{0.54} & \textit{0.92} & \textit{1.36} & 1.47   & & \textit{0.34} & \textit{0.59} & \textit{1.00} & \textit{1.15}  & & \textit{0.47} & \textit{0.81} & \textit{1.31} & \textit{1.50}   & & \textit{0.23} & \textit{0.39} & \textit{0.69} & \textit{0.81} \\ \hdashline
    Ours              & \textbf{0.45} & \textbf{0.84} & \textbf{1.27} & \textbf{1.37}   & & \textbf{0.28} & \textbf{0.53} & \textbf{0.94} & \textbf{1.08}  & & \textbf{0.44} & \textbf{0.75} & \textbf{1.24} & \textbf{1.44}   & & \textbf{0.21} & \textbf{0.37} & \textbf{0.67} & \textbf{0.79} \\ 
%    Joint-level \textit{abs.} & 0.49 & 0.85 & 1.30 & 1.41   & & 0.32 & 0.56 & 0.96 & 1.10  & & 0.49 & 0.81 & 1.28 & 1.46   & & 0.26 & 0.42 & 0.72 & 0.83 \\
    \hline
                              & \multicolumn{4}{l}{Waiting} & & \multicolumn{4}{l}{Walkingdog} & & \multicolumn{4}{l}{Walkingtogether} & & \multicolumn{4}{l}{\textit{Average}} \\ \cline{2-5}\cline{7-10}\cline{12-15}\cline{17-20}
               Milliseconds   & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400   & & 80   & 160  & 320  & 400    & & 80   & 160  & 320  & 400  \\ \toprule
        Run.-avg. 4           & 0.57 & 0.82 & 1.24 & 1.39   & & 0.74 & 0.97 & 1.27 & 1.34  & & 0.57 & 0.79 & 1.08 & 1.18   & & 0.62 & 0.86 & 1.21 & 1.34 \\ 
        Run.-avg. 2           & 0.45 & 0.71 & 1.17 & 1.32   & & 0.61 & 0.90 & 1.23 & 1.32  & & 0.46 & 0.72 & 1.05 & 1.17   & & 0.50 & 0.78 & 1.16 & 1.30 \\ 
        Zero-velocity         & 0.39 & 0.64 & 1.13 & 1.28   & & 0.53 & 0.85 & 1.20 & 1.31  & & 0.40 & 0.67 & 1.03 & 1.15   & & 0.43 & 0.72 & 1.13 & 1.28 \\ 
        GRU unsup.            & 0.42 & 0.70 & 1.25 & 1.44   & & 0.52 & 0.85 & 1.22 & 1.33  & & 0.37 & 0.60 & 0.89 & 1.00   & & 0.45 & 0.76 & 1.19 & 1.34 \\
        OuaterNet vel.        & \textit{0.32} & \textit{0.54} & \textit{1.00} & \textit{1.15}   & & \textit{0.48} & \textit{0.78} & \textit{1.12} & \textit{1.21}  & & \textit{0.28} & \textit{0.45} & \textit{0.69} & \textit{0.79}   & & \textit{0.37} & \textit{0.62} & \textit{1.00} & \textit{1.14} \\ \hdashline
    Ours               & \textbf{0.28} & \textbf{0.47} & \textbf{0.90} & \textbf{1.07}   & & \textbf{0.43} & \textbf{0.70} & \textbf{1.05} & \textbf{1.17}  & & \textbf{0.25} & \textbf{0.40} & \textbf{0.63} & \textbf{0.75}   & & \textbf{0.32} & \textbf{0.56} & \textbf{0.94} & \textbf{1.08} \\
%    Joint-level \textit{abs.} & 0.30 & 0.55 & 0.99 & 1.15   & & 0.47 & 0.74 & 1.08 & 1.20  & & 0.29 & 0.47 & 0.68 & 0.81   & & 0.36 & 0.61 & 0.98 & 1.13 \\
    \hline
    \end{tabular}
    }
\end{table}
